Testing New Scalar Interactions in Few-Electron Highly Charged Ions

We investigate how a hypothetical scalar boson mediating an interaction between electrons as well as between electrons and nucleons would affect the g factor of lithium-like highly charged ions. In such ions, the strong nuclear Coulomb fields enhance electron-electron interactions, making them ideal systems for detecting subtle new physics signatures. Exceptionally accurate quantum electrodynamic predictions and experimental data in such few-electron systems allow for sensitive probes, thereby enabling bounds on the boson's coupling strength. Exploiting the enhanced sensitivity of highly charged ions to short-range interactions, we combine g-factor measurements and quantum electrodynamic theory predictions of lithium- and hydrogen-like ions with the free-electron magnetic moment and an isotope-shift measurement to constrain simultaneously the electron-proton, electron-neutron, and electron-electron coupling combinations as functions of the scalar mass. We find that precision g-factor spectroscopy provides competitive constraints on scalar interactions over a broad mass range and, in particular, yields bounds on electron-electron interactions from bound-state QED observables.

==> name.tex <==
 \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2CMU.pdf}
        \caption{}
        \label{fig:2CMU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2DMU.pdf}
        \caption{}
        \label{fig:2DMU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2CMD.pdf}
        \caption{}
        \label{fig:2CMD}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2DMD.pdf}
        \caption{}
        \label{fig:2DMD}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2CSU.pdf}
        \caption{}
        \label{fig:2CSU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2DSU.pdf}
        \caption{}
        \label{fig:2DSU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2CSD.pdf}
        \caption{}
        \label{fig:2CSD}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/2DSD.pdf}
        \caption{}
        \label{fig:2DSD}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1CMU.pdf}
        \caption{}
        \label{fig:1CMU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1DMU.pdf}
        \caption{}
        \label{fig:1DMU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1CMD.pdf}
        \caption{}
        \label{fig:1CMD}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1DMD.pdf}
        \caption{}
        \label{fig:1DMD}
    \end{subfigure}
    %%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1CSU.pdf}
        \caption{}
        \label{fig:1CSU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1DSU.pdf}
        \caption{}
        \label{fig:1DSU}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1CSD.pdf}
        \caption{}
        \label{fig:1CSD}
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \includegraphics[width=\linewidth]{Figures/one-scalar/1DSD.pdf}
        \caption{}
        \label{fig:1DSD}
    \end{subfigure}
    \caption{All possible one-scalar exchange contributions to the $g$ factor}
